Propositional Dynamic Logic for Hyperproperties

Information security properties of reactive systems like non-interference often require relating different executions of the system to each other and following them simultaneously. Such hyperproperties can also be useful in other contexts, e.g., when analysing properties of distributed systems like linearizability. Since common logics like LTL, CTL, or the modal mu-calculus cannot express hyperproperties, the hyperlogics HyperLTL and HyperCTL* were developed to cure this defect. However, these logics are not able to express arbitrary omega-regular properties. In this paper, we introduce HyperPDL-Delta, an adaptation of the Propositional Dynamic Logic of Fischer and Ladner for hyperproperties, in order to remove this limitation. Using an elegant automata-theoretic framework, we show that HyperPDL-Delta model checking is asymptotically not more expensive than HyperCTL* model checking, despite its vastly increased expressive power. We further investigate fragments of HyperPDL-Delta with regard to satisfiability checking.

==> math/defs/HyperFO.tex <==
\begin{definition}[\cite{Finkbeiner2017a}]
Let $T \subseteq (2^{AP})^{\omega}$ be a set of traces. The relational structure $\underline{T} = (T \times \mathbb{N}, <^{\underline{T}},E^{\underline{T}}, (P^{\underline{T}}_a)_{a \in AP})$ is given by
\begin{itemize}
	\item $<^{\underline{T}} = \{(t, n), (t, n')) \mid t \in T \land n < n' \in \mathbb{N}\}$,
	\item $E^{\underline{T}} = \{(t, n), (t', n)) \mid t, t'\in T \land n \in \mathbb{N}\}$
	\item $P^{\underline{T}}_a = \{(t, n) \mid a \in t(n)\}$.
\end{itemize}
The first-order logic of hyperproperties is first-order logic over the signature $\{<, E\} \cup \{P_a \mid a \in AP\}$ with atomic equality formulas $x=y$, the predicates $E(x,y)$ and $P_a(x)$ for $a \in AP$ as well as conjunction, disjunction, negation and (universal and existential) quantification. This logic is denoted by $FO(<, E)$.
\end{definition}
The structure $\underline{T}$ represents a set of traces by $|T|$ copies of $\mathbb{N}$, where $E(x,y)$ denotes that $x$ and $y$ refer to two traces at the same point of time. 


==> math/defs/alternationdepth.tex <==
\begin{definition}[Alternation depth]
	A HyperPDL-$\Delta$ formula $\varphi$ has alternation depth $0$ plus the highest number of alternations from existential to universal and universal to existential quantifiers along any of the paths of the formula's syntax tree.
	Occurrences of quantifiers in $\alpha$ as well as $\forall$ quantifiers in the right subformula of $\langle \alpha \rangle \varphi$ and $\exists$ quantifiers in the right subformula of $[\alpha] \varphi$ count as additional alternations on these paths.
	We call a HyperPDL-$\Delta$ formula with alternation depth $0$ alternation-free.
\end{definition}

\begin{comment}
\begin{definition}[Alternation depth]
A HyperPDL-$\Delta$ formula $\varphi$ has alternation depth $0$ plus the highest number of alternations from existential to universal and universal to existential quantifiers along any of the paths of the formula's syntax tree.
Occurrences of quantifiers in particular constructs as seen in \autoref{figure:alternationdepth} count as additional alternation depth on these paths.
We call a HyperPDL-$\Delta$ formula with alternation depth $0$ alternation-free.
\end{definition}
\begin{figure}
\centering
\begin{tabular}{l l | l l}
& & $\exists$ & $\forall$ \\
\hline
$\langle \alpha \rangle \varphi$: & $\alpha$ & $\times$ & $\times$ \\
& $\varphi$ & & $\times$ \\
$[ \alpha ] \varphi$: & $\alpha$ & $\times$ & $\times$ \\
& $\varphi$ & $\times$ & \\
$\Delta \alpha$: & $\alpha$ & $\times$ & $\times$ \\
$\lnot \Delta \alpha$: & $\alpha$ & $\times$ & $\times$
\end{tabular}
\caption{Construction/Quantifier combinations increasing the alternation depth}
\label{figure:alternationdepth}
\end{figure}

\begin{definition}[Alternation depth]
A HyperPDL-$\Delta$ formula $\varphi$ has alternation depth $0$ plus the highest number of alternations from existential to universal and universal to existential quantifiers along any of the paths of the formula's syntax tree.
Occurrences of quantifiers in programs $\alpha$ as well as $\forall$ quantifiers in the right subformula of $\langle \alpha \rangle \varphi$ or $\exists$ quantifiers in the right subformula of $[\alpha]\varphi$ count as additional alternation depth.
We call a HyperPDL-$\Delta$ formula with alternation depth $0$ alternation-free.
\end{definition}

\begin{tabular}{l | l l l l l}
& $\langle \alpha \rangle \varphi$: & &	$[ \alpha ] \varphi$ & & $\Delta \alpha$: \\
& $\alpha$ & $\varphi$ & $\alpha$ & $\varphi$ $\alpha$ \\
\hline
$\exists$ & $\times$ & & $\times$ & $\times$ & $\times$ \\
$\forall$ & & $\times$ & & &
\end{tabular}
\end{comment}

==> math/proofs/complexity.tex <==
\begin{proof} of \autoref{complexity}
	
\end{proof}

==> math/proofs/complexitycorollary.tex <==
\begin{proof} of \autoref{complexitycorollary}
	
\end{proof}

==> math/proofs/hardnessalt.tex <==
\begin{proof}[Alternative proof of \autoref{hardness}]
	
	This proof is similar to the completeness proof of HyperCTL$^*$ model checking from \cite{Clarkson2014}.
	We present this alternative to a reduction from HyperCTL$^*$ model checking to reassure that our result still holds for the slightly changed notion of criticality compared to the notion of alternation depth in \cite{Clarkson2014}.
	
	We reduce the satisfiability Problem for $\Sigma_k^{QPTL}$ (QPTL formulas starting with an existential quantifier and with $k-1$ quantifier alternations) which is $NSPACE(g(k-1,n))$-complete by \cite{Sistla1987} to the model checking problem for HyperPDL-$\Delta$ formulas with criticality $k-1$.
	We will assume that a given QPTL formula $\varphi$ is in closed prenex normal form, that is $(Q_1 a_1 Q_2 a_2 ... Q_l p_l)(f)$ where $Q_i$ are quantifiers and $f$ is a quantifier free formula with only atomic propositions $p_1,...,p_l$.
	
	For the reduction we construct a $KTS$ $\mathcal{T}$ and a HyperPDL-$\Delta$ formula $\varphi'$ such that
	\begin{equation*}
		\varphi \text{ is satisfiable } \Leftrightarrow \mathcal{T} \models \varphi'
	\end{equation*}
	
	We choose $AP = \{p\}, \Sigma = \{\sigma\}$ and the $KTS$ is given as $\mathcal{T} = (\{s_0,s_1\},s_0,\{\delta_{\sigma}\}, L)$ where $\delta_{\sigma} = S \times S$ and $L(s_0) = \emptyset, L(s_1) = \{p\}$.
	Since we chose an alphabet $\Sigma$ of size $1$, we can omit programs $\sigma$ from paths in $\mathcal{T}$ and thus obtain $Paths^*(\mathcal{T},s) = (2^{AP})^{\omega}$ for $s \in \{s_0,s_1\}$.
	Thus, by slight abuse of notation, we will use traces and paths in $\mathcal{T}$ interchangeably in path assignments.
	Our HyperPDL-$\Delta$ formula $\varphi'$ is given by $tr(\varphi)$ which is constructed inductively from $\varphi$ as follows:
	\begin{align*}
		tr(p) &= \langle \bullet \rangle p_{\pi} \\
		tr(\varphi_1 \land \varphi_2) &= tr(\varphi_1) \land tr(\varphi_2) \\
		%tr(\varphi_1 \lor \varphi_2) &= tr(\varphi_1) \lor tr(\varphi_2) \\
		tr(\lnot \varphi_1) &= \lnot tr(\varphi_1) \\
		tr(X \varphi_1) &= \langle \bullet \rangle tr(\varphi_1) \\
		tr(F \varphi_1) &= \langle \bullet^* \rangle tr(\varphi_1) \\
		tr(\exists p \varphi_1) &= \exists \pi . tr(\varphi_1) %\land [\bullet\bullet^*] (p_{\pi_l} \leftrightarrow \lnot p_{\pi_{l-1}}) %\\
		%tr(\forall p_l \varphi_1) &= \forall \pi_l . tr(\varphi_1) \land [\bullet\bullet^*] (p_{\pi_l} \leftrightarrow \lnot p_{\pi_{l-1}})
	\end{align*}
	The translation $tr(\varphi)$ indeed has the desired criticality since all critical quantifiers are induced by quantifier alternation.
	
	The above claim follows straightforwardly from the statement: for all subformulas $\hat{\varphi}$ of $\varphi$ and traces $t \in (2^{AP})^{\omega}$ it holds $\overleftarrow{t} \models \hat{\varphi}$ iff $\Pi \models_{\mathcal{T}} tr(\hat{\varphi})$ for some path assignment $\Pi$ with $\Pi(\epsilon) = t$, where we use $\overleftarrow{t}$ to denote the trace $t$ shifted left by one.
	This can be shown by induction over the structure of $\hat{\varphi}$.
	%We will show this by induction over the structure of $\hat{\varphi}$.
	
	\begin{comment}
	\boldmath$\hat{\varphi} = p$\unboldmath: 
	On the one hand assume that $\overleftarrow{t} \models \hat{\varphi}$.
	
	On the other hand assume that $\Pi \models_{\mathcal{T}} \hat{\varphi}$.

	\boldmath$\hat{\varphi} = \varphi_1 \land \varphi_2$\unboldmath:
	On the one hand assume that $\overleftarrow{t} \models \hat{\varphi}$.
	
	On the other hand assume that $\Pi \models_{\mathcal{T}} \hat{\varphi}$.
	
	\boldmath$\hat{\varphi} = \lnot \varphi_1$\unboldmath:
	On the one hand assume that $\overleftarrow{t} \models \hat{\varphi}$.
	
	On the other hand assume that $\Pi \models_{\mathcal{T}} \hat{\varphi}$.
	
	\boldmath$\hat{\varphi} = X \varphi_1$\unboldmath:
	On the one hand assume that $\overleftarrow{t} \models \hat{\varphi}$.
	
	On the other hand assume that $\Pi \models_{\mathcal{T}} \hat{\varphi}$.
	
	\boldmath$\hat{\varphi} = F \varphi_1$\unboldmath:
	On the one hand assume that $\overleftarrow{t} \models \hat{\varphi}$.
	
	On the other hand assume that $\Pi \models_{\mathcal{T}} \hat{\varphi}$.
	
	\boldmath$\hat{\varphi} = \exists p \varphi_1$\unboldmath:
	On the one hand assume that $\overleftarrow{t} \models \hat{\varphi}$.
	
	On the other hand assume that $\Pi \models_{\mathcal{T}} \hat{\varphi}$.
	\end{comment}
	


	
	\hfill\qed
\end{proof}


==> math/proofs/linearstructures.tex <==
\begin{proof}
On singleton trace sets, we can remove all quantifiers from HyperLTL and HyperCTL* formulas for any formula $\phi$ since all quantifiers then refer to the same trace. Therefore, these logics become semantically equivalent to LTL here. Furthermore, by Kamp's Theorem \cite{Kamp1968}, $FO(<)$ is equivalent to LTL on linear structures. It is well-known \cite{Wolper1983} that LTL cannot specify that an atomic proposition may only occur on even indices. In contrast, HyperPDL-$\Delta$ can obviously do so.
\hfill\qed
\end{proof}


==> math/theorems/HyperCTLStar.tex <==
\begin{theorem}\label{HyperCTLStar}
\begin{itemize}$ $
	\item HyperCTL$^* <$ HyperPDL-?
	\item  $HyperCTL^*$ and Hyper-PDL without ? are incomparable
\end{itemize}
\end{theorem}

\begin{proof}(Sketch)	
	The embedding is immediate. For a deterministic LTS, we obtain that every HyperCTL$^*$ formula is equivalent to an LTL formula. However, LTL cannot count modulo $k$ for any $k$, while $HyperPDL-?$ can.
	\hfill\qed
\end{proof}


==> math/theorems/HyperFO.tex <==
\begin{theorem}\label{HyperFO}
HyperFO and all HyperPDL-fragments are incomparable.
\end{theorem}


==> math/theorems/PDLembedding.tex <==
\begin{theorem}
For every PDL$-\Delta$ formula $\phi$, there is a HyperPDL$-\Delta$ formula $\phi'$ such that for all $KTSs$ $\mathcal{T}$, $\mathcal{T} \models \phi \iff \mathcal{T} \models \phi'$ holds.
\end{theorem}


==> math/theorems/complexitycorollary.tex <==
\begin{corollary}\label{complexitycorollary}
	The model checking problem for the alternation-free fragment of HyperPDL is PSPACE-complete in the size of the formula and NLOGSPACE-complete in the size of the Kripke transition system.
\end{corollary}

\begin{proof}(Sketch)
	The upper bound is a direct corollary of \autoref{complexity}.
	The lower bound is obtained by a reduction from HyperLTL model checking.
	\hfill\qed
\end{proof}

==> math/theorems/etlasatisfiability.tex <==
\begin{theorem}[\cite{Kupferman2001}]
	$ETL_a$ satisfiability checking is PSPACE-complete.
\end{theorem}

==> math/theorems/increasedpower.tex <==
\begin{corollary}
$\text{HyperCTL}^* < $ $HyperPDL$-$\Delta$
\end{corollary}


==> math/theorems/linearstructures.tex <==
\begin{comment}
\begin{figure}[h!]
	\footnotesize
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1em,
                    semithick]

  \node[label=below:{$1$}] (A)                    {$p$};
  \node[label=below:{$2$}]         (B) [right = of A] {$p$};
  \node[]         (C) [right = of B] {\dots};
  \node[label=below:{$i$}]         (D) [right = of C] {$\neg p$};
  \node[label=below:{$i+1$}]         (E) [right = of D] {$p$};
  \node[]         (F) [right = of E] {\dots};
	\path (A) edge              node {} (B);
	\path (B) edge              node {} (C);
	\path (C) edge              node {} (D);
	\path (D) edge              node {} (E);

\end{tikzpicture}
\caption{The structure $S_i$}
\label{figure:path}
\end{figure}
\end{comment}
\begin{theorem}${}$
$HyperLTL = HyperCTL^* = FO(<, E) = FO(<)= LTL$ and  $LTL < HyperPDL-\Delta$ on linear structures, i.e. structures with only one path.
\end{theorem}

\input{math/proofs/linearstructures}

